Neural Network Interatomic Potentials For Open Surface Nano-mechanics Applications

Material characterization in nano-mechanical tests requires precise interatomic potentials for the computation of atomic energies and forces with near-quantum accuracy. For such purposes, we develop a robust neural-network interatomic potential (NNIP), and we provide a test for the example of molecular dynamics (MD) nanoindentation, and the case of body-centered cubic crystalline molybdenum (Mo). We employ a similarity measurement protocol, using standard local environment descriptors, to select ab initio configurations for the training dataset that capture the behavior of the indented sample. We find that it is critical to include generalized stacking fault (GSF) configurations, featuring a dumbbell interstitial on the surface, to capture dislocation cores, and also high-temperature configurations with frozen atom layers for the indenter tip contact. We develop a NNIP with distinct dislocation nucleation mechanisms, realistic generalized stacking fault energy (GSFE) curves, and an informative energy landscape for the atoms on the sample surface during nanoindentation. We compare our NNIP results with nanoindentation simulations, performed with three existing potentials -- an embedded atom method (EAM) potential, a gaussian approximation potential (GAP), and a tabulated GAP (tabGAP) potential -- that predict different dislocation nucleation mechanisms, and display the absence of essential information on the shear stress at the sample surface in the elastic region. We believe that these features render specialized NNIPs essential for simulations of nanoindentation and nano-mechanics with near-quantum accuracy.

==> macros_junk.tex <==
%%% legend square
\newcommand{\legSq}[5]{%(xc,yc,color,text,offset)
                \coordinate (a) at (0,0); % reference
                \node[white] at (a) {\tiny.};               %   
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
				 \draw[#3,fill] ($(b)-(0.0,0.075)$) rectangle ($ (d) + (0.0,0.075) $); % 2*0.075 square length
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		    \node at ($(center1)+(#5,0)$) {{\color{black}#4}}; %text
}
%%% legend square
\newcommand{\legSqNoFill}[3]{
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
				 \draw[#3] ($(b)-(0.0,0.075)$) rectangle ($ (d) + (0.0,0.075) $); % 2*0.075 square length
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
}
%%% legend square
\newcommand{\legSqTxt}[3]{
		\begin{tikzpicture}
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
				 \draw[#3,fill=#3] ($(b)-(0.0,0.075)$) rectangle ($ (d) + (0.0,0.075) $); % 2*0.075 square length
 %               \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
 %               \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}
%%% legend circle
\newcommand{\legCirc}[5]{%(xc,yc,color,text,offset)
                \coordinate (a) at (0,0); % reference
                \node[white] at (a) {\tiny.};               %   
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw[#3] (center1) circle (2pt);
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		    \node at ($(center1)+(#5,0)$) {{\color{black}#4}}; %text
}
%%% legend circle
\newcommand{\legFilledCirc}[3]{
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw[#3,fill] (center1) circle (2pt);
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
}

%%% legend circle
\newcommand{\legFilledStar}[3]{
            \tikzstyle{scorestars}=[star, star points=5, star point ratio=2.25, draw, inner sep=1.3pt, anchor=outer point 3]%
		\begin{tikzpicture}
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw (#1,#2) node[name=star, scorestars, fill=#3] {};

		\end{tikzpicture}		
}

%%% legend circle
\newcommand{\circTxtFill}[3]{
		\begin{tikzpicture}
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw[#3,fill=#3] (center1) circle (2pt);
		\end{tikzpicture}		
}

%%% legend circle
\newcommand{\legCircTxt}[3]{
		\begin{tikzpicture}
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw[#3] (center1) circle (2pt);
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}
%%% legend diamond
\newcommand{\legDiamond}[3]{
			     \coordinate (center1) at (#1,#2); % centeroid
                \coordinate (b) at ($ (center1) + (0.075,0.0) $); % L=.2
                \coordinate (c) at ($ (center1) + (0,0.075) $); 
                \coordinate (d) at ($ (center1) + (-0.075,0) $);
                \coordinate (e) at ($ (center1) + (0.0,-0.075) $);
				 \draw[#3] (b) -- (c) -- (d) -- (e) -- (b);
                \coordinate (c) at ($ (b) + (.1,0) $); %0.5*0.9/2
                \coordinate (e) at ($ (d) - (.1,0) $); %0.5*0.9/2
                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
}
%%% legend diamond
\newcommand{\legDiamondTxt}[3]{
		\begin{tikzpicture}
			     \coordinate (center1) at (#1,#2); % centeroid
                \coordinate (b) at ($ (center1) + (0.075,0.0) $); % L=.2
                \coordinate (c) at ($ (center1) + (0,0.075) $); 
                \coordinate (d) at ($ (center1) + (-0.075,0) $);
                \coordinate (e) at ($ (center1) + (0.0,-0.075) $);
				 \draw[#3,fill=#3] (b) -- (c) -- (d) -- (e) -- (b);
                \coordinate (c) at ($ (b) + (.1,0) $); %0.5*0.9/2
                \coordinate (e) at ($ (d) - (.1,0) $); %0.5*0.9/2
%                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
%                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}
%%% legend triangle up
\newcommand{\legTriangle}[3]{
			     \coordinate (center1) at (#1,#2); % centeroid
                \coordinate (b) at ($ (center1) - 0.17*(0.5,0.289) $); % L=.2
                \coordinate (c) at ($(center1) + 0.17*(0.5,-0.289) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + 0.17*(0,0.366) $);
%				 \draw[#3] (b) -- (c) -- (d) -- (b);
				\filldraw[draw=#3, fill=#3, line width=0.1mm] %,densely dotted] 
%    (b) to[out=300, in=130] (c) -- (d) -- cycle;                 
    (b) -- (c) -- (d) -- cycle;                 
    			\coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
                \draw[#3,fill][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3,fill][line width=0.1mm] (d) -- (e); % vertical line
    }                
\newcommand{\legTriangleTxt}[3]{
		\begin{tikzpicture}
			     \coordinate (center1) at (#1,#2); % centeroid
                \coordinate (b) at ($ (center1) - 0.17*(0.5,0.289) $); % L=.2
                \coordinate (c) at ($(center1) + 0.17*(0.5,-0.289) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + 0.17*(0,0.366) $);
%				 \draw[#3] (b) -- (c) -- (d) -- (b);
				\draw[black,fill=#3, line width=0.1mm] %,densely dotted] 
%    (b) to[out=300, in=130] (c) -- (d) -- cycle;                 
    (b) -- (c) -- (d) -- cycle;                 
    			\coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
%                \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
%                \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}		
		
%%% filled circle
\definecolor{light-gray}{gray}{0.85}
\newcommand{\filledCirc}[4]{
		\begin{tikzpicture}
                \coordinate (center1) at (#1,#2); % center of figure
				 \draw[fill=#3] (center1) circle (2pt);
				 \draw[color=#4,line width=0.05mm] (center1) circle (2pt);
		\end{tikzpicture}		
}
 			     %% legend left triangle
\newcommand{\leftTriang}[3]{
		\begin{tikzpicture}
			     \coordinate (center1) at (#1,#2); % center of figure 382
                \coordinate (b) at ($ (center1) + 0.17*(0.289,0.5) $); % L=.2
                \coordinate (c) at ($ (center1) + 0.17*(0.289,-0.5) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + 0.17*(-0.366,0.0) $);
				 \draw[fill=#3,#3] (b) -- (c) -- (d) -- (b);
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
%               	 \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
%                	\draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}
				 %%  legend triangle down
\newcommand{\downTriang}[3]{
			     \coordinate (center1) at (#1,#2); % centeroid
               \coordinate (b) at ($ (center1) - 0.17*(0.5,-0.289) $); % L=.2
                \coordinate (c) at ($ (center1) + 0.17*(0.5,+0.289) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) - 0.17*(0,0.366) $);
				\filldraw[draw=#3, fill=#3, line width=0.1mm] %,densely dotted] 
    (b) -- (c) -- (d) -- cycle;              
                    \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
                \draw[#3,fill][line width=0.1mm] (b) -- (c); % vertical line
                \draw[#3,fill][line width=0.1mm] (d) -- (e); % vertical line
}

\newcommand{\rightTriang}[3]{
		\begin{tikzpicture}
				 %% 2nd legend triangle right
			    \coordinate (center1) at (#1,#2); % centeroid
                \coordinate (b) at ($ (center1) + 0.17*(-0.289,0.5) $); % L=.2
                \coordinate (c) at ($ (center1) + 0.17*(-0.289,-0.5) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + 0.17*(0.366,0.0) $);
				 \draw[black,fill=#3] (b) -- (c) -- (d) -- (b);
                \coordinate (b) at ($ (center1) - (.075,0) $);
                \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
 %               \draw[gray][line width=0.1mm] (b) -- (c); % vertical line
 %               \draw[gray][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
 }
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  draw slope
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\drawSlope}[7]{ %(xc,yc,a,theta,color,text)
				\coordinate (center1) at (#1,#2); % center of figure
				 \FPeval{\nx}{cos(#4*pi/180)}%
				 \FPeval{\ny}{sin(#4*pi/180)}%
				 \FPeval{\absNx}{abs(\nx)}%
				 \FPeval{\absNy}{abs(\ny)}%
%
				\coordinate (b) at ($ (center1) + #3*(-\ny,+\nx) $);
				\coordinate (c) at ($ (center1) - #3*(-\ny,+\nx) $); 
%
				 \FPeval{\xx}{(-\nx*\ny)}%
				\ifdim\xx pt < 0pt 
				\coordinate (d) at ($ (c) -2*#3*\ny*(1,0) $);
%				\node at ($(d) +(0,#3*\nx)-0.2*(\nx/\absNx,0)$) {{\color{#5}$#6$}}; % 1 (d,b,c)
				\node at ($(d) +(0,#3*\nx)-0.2*(\nx/\absNx,0)$) {{\color{#5}#6}}; % 1 (d,b,c)
				\node at ($(d)+(#3*\ny,0)-0.15*(0,\ny/\absNy)$) {{\color{#5}\vspace{-12pt}#7}}; %2
				\else
				\coordinate (d) at ($ (c) +2*#3*\nx*(0,1) $);
%				\node at ($(d)-#3*\nx*(0,1)-0.2*\nx/\absNx*(1,0)$) {{\color{#5}$#6$}}; % 1
				\node at ($(d)-#3*\nx*(0,1)-0.2*\nx/\absNx*(1,0)$) {{\color{#5}#6}}; % 1
				\node at ($(d)-#3*\ny*(1,0)-0.15*\ny/\absNy*(0,1)$) {{\color{#5}\vspace{-12pt}#7}}; %2
				\fi
%
				\draw[#5,line width=0.1mm] (d) -- (b); % horizontal line
				\draw[#5,line width=0.1mm] (d) -- (c); % vertical line
				\draw[#5,line width=0.1mm] (b) -- (c); % vertical line
} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  scale bar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\scaleBar}[8]{%(xc,yc,l,t,scale0,scale1,scale2,text)
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (#3,#4/2) $); %l=0.4
                \coordinate (d) at ($ (center1) + (#3,#4/2) $);
				 \draw[black,fill] ($(b)$) rectangle ($(d)$); % 2*0.075 square length

				\node at ($(b)-(0,#4)$){{\color{black}\tiny $#5$}};
				\node at ($(b)+(2*#3,-#4)$) {{\color{black}\tiny $ #6$}};
				\node at ($(b)+(2*#3,+2.6*#4)$) {{\color{black}$\scriptstyle\text{#8}$}}; % 1
			     \coordinate (center2) at ($ (center1) + 2*(#3,0.0)$);  % l=0.4
                \coordinate (b) at ($ (center2) - (#3,#4/2) $);
                \coordinate (d) at ($ (center2) + (#3,#4/2) $);
				 \draw[black] ($(b)$) rectangle ($(d)$); % 2*0.075 square length
				\node at ($(d)-(0,5*#4)$) {{\color{black}\tiny $#7$}};		
				}	
				
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  scale bar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\scaleBarr}[8]{%(xc,yc,l,t,scale0,scale1,scale2,text)
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (#3,#4/2) $); %l=0.4
                \coordinate (d) at ($ (center1) + (#3,#4/2) $);
				 \draw[black,fill] ($(b)$) rectangle ($(d)$); % 2*0.075 square length

				\node at ($(b)-(0,#4)$){{\color{black} $#5$}};
				\node at ($(b)+(2*#3,-#4)$) {{\color{black} $ #6$}};
				\node at ($(b)+(2*#3,+2.6*#4)$) {{\color{black}$\text{#8}$}}; % 1
			     \coordinate (center2) at ($ (center1) + 2*(#3,0.0)$);  % l=0.4
                \coordinate (b) at ($ (center2) - (#3,#4/2) $);
                \coordinate (d) at ($ (center2) + (#3,#4/2) $);
				 \draw[black] ($(b)$) rectangle ($(d)$); % 2*0.075 square length
				\node at ($(d)-(0,2*#4)$) {{\color{black} $#7$}};		
				}	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  coordinate system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\coordSys}[9]{%(xo,yo,l,x1,y1,x2,y2,x3,y3)	
    	                 % draw arrow
			\coordinate (center2) at (#1,#2); % center of figure
            \coordinate (x1) at ($ (center2) + #3*(#4,#5) $); % length=0.4
            \coordinate (x2) at ($ (center2) - .3*#3*(#4,#5) $); % length=0.4
            \coordinate (y1) at ($ (center2) + #3*(#6,#7) $);
            \coordinate (y2) at ($ (center2) - .3*#3*(#6,#7) $);
            \coordinate (z1) at ($ (center2) + #3*(#8,#9) $); %arrow length
            \coordinate (z2) at ($ (center2) - .3*#3*(#8,#9) $); %arrow length
            \draw[->,>=stealth,black][line width=0.4mm] (x2) -- (x1);
			\node at ($(x1)+(0.2,0)$){{\color{black} \large $x$}};
            \draw[->,>=stealth,black][line width=0.4mm] (y2) -- (y1);
            \node at ($(y1)+(0,0.2)$){{\color{black} \large $y$}};
            \draw[->,>=stealth,black][line width=0.4mm] (z2) -- (z1);
			\node at ($(z1)+(0,0.2)$){{\color{black} \large $z$}};
    	}
    	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  coordinate system
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\newcommand{\coordSysTwoDim}[7]{%(xo,yo,l,x1,y1,x2,y2)	
    	                 % draw arrow
			\coordinate (center2) at (#1,#2); % center of figure
            \coordinate (x1) at ($ (center2) + #3*(#4,#5) $); % length=0.4
            \coordinate (x2) at ($ (center2) - .3*#3*(#4,#5) $); % length=0.4
            \coordinate (y1) at ($ (center2) + #3*(#6,#7) $);
            \coordinate (y2) at ($ (center2) - .3*#3*(#6,#7) $);
            %arrow length
            \draw[->,>=stealth,black][line width=0.4mm] (x2) -- (x1);
			\node at ($(x1)+(0.2,0)$){{\color{black} \large $x$}};
            \draw[->,>=stealth,black][line width=0.4mm] (y2) -- (y1);
            \node at ($(y1)+(0,0.2)$){{\color{black} \large $y$}};
            }
%%%%%%% vertical arrow 
\newcommand{\arrow}[3]{ %{xc,yc,txt}
            \coordinate (a) at (0,0); % reference
            \node[white] at (a) {\tiny.};               %   
            % draw arrow
			\coordinate (center2) at (#1,#2); % center of figure
            \coordinate (b) at ($ (center2) + .1*(1,0) $); % length=0.4
            \coordinate (c) at ($ (center2) - .1*(1,0) $);
            \draw[red][line width=0.2mm] (c) -- (b); % horizontal line
            \coordinate (d) at ($ (center2) - .5*(0,1) $); %arrow length
            \draw[->,>=stealth,red][line width=0.2mm] (center2) -- (d); % horizontal line
		    \node at ($(center2)+(0.0,0.15)$) {{\color{red}$\scriptstyle #3$}}; %2
}
%%% legend square
\newcommand{\legRectTxt}[3]{
		\begin{tikzpicture}
			     \coordinate (center1) at (#1,#2); % center of figure
                \coordinate (b) at ($ (center1) - (.075,0) $);
                % \coordinate (c) at ($ (b) - (.1,0) $); %0.5*0.9/2
                \coordinate (d) at ($ (center1) + (.075,0) $);
                % \coordinate (e) at ($ (d) + (.1,0) $); %0.5*0.9/2
				 \draw[black,fill=#3] ($(b)-3*(0.1,0.02)$) rectangle ($ (d) + 3*(0.1,0.02) $); % 2*0.075 square length
 %               \draw[#3][line width=0.1mm] (b) -- (c); % vertical line
 %               \draw[#3][line width=0.1mm] (d) -- (e); % vertical line
		\end{tikzpicture}		
}

==> sections/Introduction.tex <==
\section{\label{sec:introduction}Introduction}
The mechanical properties of metals and multi-component alloys are of significant 
interest in extreme operating environments. Nanoindentation techniques have been 
employed to explore, 
both experimentally and computationally, several of these 
properties including hardness, strength, and dislocation dynamics \cite{durst, 
MaierKiener2017, CASALS200755, PhysRevB.67.245405, SWADDIWUDHIPONG20061117, 
DOMINGUEZGUTIERREZ2021141912}. High and low temperature nanoindentation tests are 
specifically employed to examine the common mechanisms occurring in materials 
under extreme conditions, including dislocation nucleation, defect density, grain 
boundary effects, and junction formation, through both simulations and 
experiments \cite{article, PhysRevB.76.165422, VOYIADJIS2012205, plummer}. These 
complex mechanisms can be analyzed through the use of Molecular 
Dynamics (MD) simulations, which provide valuable information about the 
mechanical properties of the indented sample, despite the limited nanoscale depth 
range probed \cite{PhysRevLett.109.075502, SATO2019280, 
Dom_nguez_Guti_rrez_2021}. 

Realistic MD that can capture the behavior of solids during nano-indentation requires
well-developed interatomic potentials. 
Quantum mechanical simulations based on Density Functional Theory (DFT),
a powerful and well established   theoretical framework in materials properties computation 
\cite{PhysRev.136.B864, PhysRev.140.A1133},
provide the relative 
total energy and atomic forces of a given configuration, 
but are limited in scope due to their computational cost. 
NNIPs can deliver comparable accuracy to DFT but at a much lower computational cost, allowing for simulations that can capture extended systems such as those required to model nano-indentation. 

The use of machine learning (ML) methods is widespread in materials modeling~\cite{Chandrasekaran2019, PhysRevLett.120.145301, PhysRevB.97.094106, PhysRevB.97.195424, Cooper2020, Zong2018, 201900808, Nyshadham2019, Kostiuchenko2019, Deng2019, Schmidt2019, aav6490}, 
including the development of interatomic potentials~\cite{PhysRevLett.98.146401, PhysRevLett.104.136403, THOMPSON2015316, 15M1054183, PhysRevB.97.184307, PhysRevLett.120.143001, doi:10.1063/1.4966192, Shaidu2021, LI2021100359}. 
The selection of an appropriate training dataset is a crucial factor for the success of the potential, in addition to the specific ML approach 
and the atomic environment descriptors employed. 
The choice of training dataset affects the applicability of the resulting interatomic potential to different simulation scenarios. Shaidu {\em et al.}~\cite{Shaidu2021} demonstrated this point by presenting a systematic approach for creating a training dataset to develop interatomic potentials for diamond, graphite, graphene, and amorphous carbon structures. The approach used an evolutionary algorithm to sample a wide range of structures and a clustering algorithm to filter and retain only novel structures for the training dataset. The resulting potential achieved DFT-level accuracy for elastic and vibrational properties. 
Another approach to creating the training dataset is through active learning methods~\cite{Vandermause2020}. 
For instance, Vandermause {\em et al.}~\cite{Vandermause2022} used the internal uncertainties of a Gaussian process regression model during a MD simulation of a H/Pt(111) surface at high temperatures to evaluate whether
additional {\em ab-initio} 
structures were needed in the training dataset. 
The autonomous and precise way of 
constructing the training dataset lead to excellent results for the hydrogen reaction with Pt surfaces when compared to both experimental and 
DFT data.

In nanoindentation, 
often used to investigate mechanical 
properties at the nanoscale~\cite{SCHUH200632,VARILLAS2017431,KURPASKA2022110639,PATHAK20151,cryst7100321},
a small, sharp tip is pressed into the surface of a sample to 
measure the force required, and the resulting displacement into the 
material. A \textit{pop-in} event, that defines 
the transition from elastic to plastic deformation,
is produced as the indenter tip starts to penetrate the surface and 
is often used as a reference point for analyzing the mechanical behavior of a 
material, as it can provide insight into the internal structure of the sample. 
This gives the opportunity to explore the mechanisms of plastic deformation 
initiation responsible for modification of mechanical properties of the material~\cite{REMINGTON2014378,GAGEL2016399}.

Simulation of nano-indentation involves complex atomic environments including many types of crystal defects, such as stacking faults, edge and screw dislocations, 
dislocation loops, self-interstitials, and vacancies. 
In high-temperature simulations, 
the complexity of the atomic environments
increases, which is
an important factor for investigating the 
mechanical properties of materials in extreme environments. Consequently, 
to simulate such processes it is 
necessary to construct 
an interatomic potential that covers a very broad range of atomic structures  
likely to occur during modeling of the nanoindentation process through MD simulations. 
This includes surfaces, which provide information on pileup 
patterns, atoms under the tip that provide information on plastic regions, point 
defects and dislocation cores and junctions. 
Thus, the  
training dataset
is crucial for the success of these simulations, 
as it can 
affect the applicability of the resulting interatomic potential to different scenarios.

In this paper, we present a study that aims at evaluating the accuracy of a Neural 
Network interatomic potential developed using an improved random dataset from 
literature~\cite{dataset} within the PANNA (Properties from Artificial Neural Network Architectures) framework~\cite{panna}. 
We compare the 
Behler-Parrinello descriptor vectors~\cite{PhysRevLett.98.146401} of the training 
dataset with those of a single crystal BCC Molybdenum configuration, indented 
with an Embedded atom model (EAM) potential~\cite{ESalonen_2003}, to determine 
how closely the training dataset resembles the indentation process. 
To improve 
the accuracy of the potential, we introduce high 
temperature configurations with a frozen layer and generalized stacking fault 
(GSF) configurations with an interstitial on the gamma surface. These 
configurations are designed to closely mimic atoms in the dislocation cores, on 
the surface, and under the indenter tip. Our results show that including these 
configurations in the training dataset reduces the distance between the atoms in 
the training dataset and the indented sample. Finally, 
we present the results of an MD nanoindentation simulation using
the potential trained with
the modified dataset.

==> sections/Methods_and_Materials.tex <==
\section{\label{sec:Methods and Material}Methods}

%\subsection{Dataset description}

%The aim of this study is to develop a NNIP which specifically is fit for molecular dynamics nanoindnetaion simulation of BCC metals. For this reason, a Mo dataset is obtained from a recent work of Byggmästar et. al. \cite{dataset}, which is designed for extreme operational condition simulations and in the Gaussian approximation potential framework \cite{PhysRevLett.104.136403}. This dataset includes different types of configurations such as, BCC, HCP, BCC surface (100, 110, 111, 112) and point defect (vacancies and self-interstitials) unit/super cells, shown in Table.~\ref{T_1}. The number of configurations for each structure type in the original dateset ($N_s$), the number of atoms per each structure ($N_{atoms}$) and the number of selected configurations for our work ($N_{selected}$) is shown in Table.~\ref{T_1}.

\subsection{Descriptor parameters}

In this work, PANNA: Properties from Artificial Neural 
Network Architectures~\cite{panna}, which utilizes Tensorflow~\cite{tensorflow2015-whitepaper} to train/evaluate fully-connected feed-forward NNIPs, is used to develop the interatomic potential, with 
the modified version of Behler–Parrinello (mBP) descriptors~\cite{C6SC05720A, PhysRevLett.98.146401}.  
The mBP representation generates a fixed-size vector (the G-vector) for each atom in each configuration of the dataset. Each G-vector describes the environment of the corresponding atom of the configuration to which it belongs, up to a cutoff radius $R_c$. Although higher dimensional G-vectors lead to a more accurate representation of the target potential energy surface, oversized ones increase the MD simulation computational cost. In terms of the distances $R_{ij}$ and $R_{ik}$ of the atom $i$ from  its neighbors $j$ and $k$ and the angle subtended by those distances $\theta_{ijk}$, the radial and angular G-vectors are given by:


%%% Equiation 2
\begin{equation}
        G^{rad}_{i}[s]= \sum_{i\neq j} e^{-\eta (R_{ij} - R_s)^2}f_c(R_{ij})
\label{eq:G-1}
\end{equation}
%%% Equiation 2
%%% Equiation 3
\begin{equation}
\begin{split}
G^{ang}_{i}[s]&=2^{1-\zeta} \sum_{j,k\neq i} [1+cos(\theta_{ijk} - \theta_s)]^\zeta
        \\
    &\times e^{-\eta[\frac{1}{2}(R_{ij} + R_{ik})-R_s]^2}
%        \\
%    &\times 
    f_c(R_{ij}) f_c(R_{ik})
\end{split}
\label{eq:G-2}
\end{equation}
%%% Equation 3
where the smooth cutoff function (which includes the cutoff radius $R_c$) is given by:
%%% Equiation 1
\begin{equation}
f_c(R_{ij})= 
    \begin{cases}
    \frac{1}{2}\left [\cos\left (\frac{\pi R_{ij}}{R_c}\right )+1\right ], & R_{ij} \leq R_c\\
    0,   &   R_{ij} > R_c
    \end{cases}
\label{eq:G-3}
\end{equation}
%%% Equiation 1
and \(\eta\), \(\zeta\), \(\theta_s\) and $R_s$ are parameters, different for the radial and angular parts. Table.~\ref{tab:T_4} shows all values selected for the descriptor parameters in this study.
The choice of the cutoff value is made so that it covers up to three nearest neighbours of the center atom in the BCC Mo, which has a lattice constant of $a = 3.17$ \AA, and thus the third nearest neighbour's distance is $a\times\sqrt{2} = 4.48$ \AA. The length of the G-vector for a single element system is 
\begin{equation} |G_{i}[s]| = (R_s^{ang} \times \theta_s) + R_s^{rad}, 
\end{equation}
which leads to a G-vector of length 152, given the parameters reported in Table.~\ref{tab:T_4}. 

%%%%%%%%%%% Table 4
\begin{table}[bh!]
\centering
\caption{Values of the parameters that appear in the definition of the radial and angular G-vectors, Eq.s\eqref{eq:G-1}, 
\eqref{eq:G-2}, \eqref{eq:G-3}.
Where a number of components is given, the values are equispaced.}
\label{tab:T_4}
%\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{llc}
\hline
Descriptor parameter & Symbol & Value \\
\hline
\textbf{Radial component:}      &                 & \\
Radial exponent (\AA$^{-2}$)       & $\eta^{rad}$ & $32$\\
cutoff (\AA)                  & $R_c^{rad}$  & $5$\\
Number of $R_s$ radial          & $R_s^{rad}$  & $24$\\
\textbf{Angular component:}     &                 &\\
Radial exponent (\AA$^{-2}$)       &$\eta^{ang}$ & $16$\\
cutoff (\AA)                  &$R_c^{ang}$  & $5$\\
Number of $R_s$ angular         &$R_s^{ang}$  & $8$\\
Angular exponent                &$\zeta$          & $128$ \\
Number of $\theta_s$            &$\theta_s$       & $16$\\
\hline
\end{tabular}
%}
\end{table}
%%%%%%%%%%%%% table 4


%The G-vector's components are shown in Fig.~\ref{fig:Gvectors}. The top panel shows the gaussians (24 of them) for a center atom i in the radial component, while the next two panels represent the same concept for the radial and angular part of the angular component (16 and 8, respectively). The overlap of gaussians in this figure ensures that an atom's local environment is informatively described.

%\begin{figure}
%  \centering
%  \includegraphics[width=0.48\textwidth]{Figs/Gs.png}
%  \caption{An illusration of G-vector components.} 
%  \label{fig:Gvectors}
%\end{figure}

\subsection{Similarity measurements}

%\begin{figure}
%  \centering
%  \includegraphics[width=0.48\textwidth]{Figs/Good_dist.png}
%  \caption{Distribution of minimum distance of atoms in the dataset from each other and to the indneted configuration.} 
%  \label{fig:Good_dist}
%\end{figure}

%\begin{figure*}[t]
%  \centering
%  \includegraphics[width=0.70\textwidth]{Figs/ImshowDistances.png}
%  \caption{Average of minimum distances between different configuration types as well as indented samples} 
%  \label{fig:Imshow}
%\end{figure*}

In this study, a distance-based criterion is utilized to quantify the similarity between two distinct configurations. This criterion is subsequently extended to evaluate the closeness of two disparate datasets to one another. Consider two configurations, labeled as $\alpha$ and $\beta$, with $n$ and $m$ atoms per supercell, respectively. The distance matrix for the two configurations, \textbf{$D^{\alpha\beta}$}, has a $n \times m$ dimension and each element of the matrix is the eucleadian distance of atom $i$ in $\alpha$ to atom $j$ in $\beta$:

\begin{equation}
 D^{\alpha\beta}_{i,j} = \norm{G^{\alpha}_{i}[s] - G^{\beta}_{j}[s]}_2
\label{Distance}
\end{equation}

Where $i$ $\in$ $\displaystyle \{1, 2, \dots, n \}$ and $j$ $\in$ $\displaystyle \{1, 2, \dots, m \}$, and each $G[s]$ is a 152 dimensional vector, as explained in the previous section. The minimum value of each row in the distance matrix, \textbf{$\min \{D^{\alpha\beta}_{i,:}\}$}, corresponds to a $n$-dimensional vector, $d^{\alpha\beta}$, with each element ($d^{\alpha\beta}_{i,J}$) corresponding to the closest \emph{unique} atom $J$ in $\beta$ to atom $i$ in $\alpha$:

\begin{equation}
\textbf{$D^{\alpha\beta}$}=\left[
\begin{array}{ccc}
   d^{\alpha\beta}_{1,1} & \cdots & d^{\alpha\beta}_{1,m} \\
   \vdots & \vdots& \vdots \\
   d^{\alpha\beta}_{n,1} & \cdots & d^{\alpha\beta}_{n,m}
\end{array}
\right] \xrightarrow{\min \{D^{\alpha\beta}_{i,:}\}} d^{\alpha\beta}=\left[
\begin{array}{c}
   d^{\alpha\beta}_{1,J}\\
   \vdots\\
   d^{\alpha\beta}_{n,J}
\end{array}
\right]
\end{equation}

Having the values in $d^{\alpha\beta}$, we can evaluate what is the \emph{largest minimum} distance of, for example, atom $i$ in $\alpha$ from all the atoms in $\beta$. In other words, using this tool we can find the pair of atoms in two separate configurations that have the most similar local atomic environments. This means, the final $d^{\alpha\beta}$ for two identical configurations should be a vector with all the elements equal to zero. The same outcome will occur upon rotating the cell and/or permuting two atoms with the same type, in one of the identical configurations, due to the inherent invariances within the mBP formalism.

Following the  "similarity measurement" idea presented in this section, we can define a distance matrix \textbf{$D^{AB}$} for two independent datasets $A$ and $B$, consisting of $M$ and $N$ atoms per dataset. In our case, we used this concept to decide how far an indented configuration is from an initial dataset. We then added/removed peculiar configurations to/from the dataset so that it best serves our needs.

This methodology is useful because, the final NNIP is used as the following for a MD simulation: at each MD step, the G-vector for each atom in the simulation cell is calculated and the corresponding energy and forces will be estimated from the network. Therefore, the closer the NNIP's training set is to the simulation dynamics, the more accurate the predicted energy and forces will be compared to DFT.

%This methodology is useful because, after training the NNIP, the final interatomic potential can be used in nanoindentation MD simulations to calculate the G-vectors of atoms in the simulation cell. Based on these G-vectors as the input features of the neural network model, the energies and forces of corresponding atoms can be predicted from the network. This approach has an added advantage in that it can be used to verify if a given dataset accurately represents the entire MD simulation for which an interatomic potential was trained and determine if additional data is required to improve the potential.
%The "reasonable" threshold distance in this study is defined as the maximum of the minimum distances of the atoms in the dataset to each other, shown in Fig.~\ref{fig:Good_dist}. Since our study's goal is to develop an interatomic potential for nanoindnetation simulations, the distribution of the minimum distances of atoms of an indented configuration (acquired using an EAM potential) with a crystal orientation of $x=[100]$, $y=[010]$ and $z=[001]$ and the dimentions if $9.44 nm\times 9.76 nm\times8.49 nm$ to the atoms in the dataset is also shown and the maximum distance, before the start of the distribution's tail (which is 6 \AA), is chosen as a threshold in this work. The nanoindentation simulation details is going to be further explained.

%In order to get a sense of, and analyse the dataset, the average of the minimum distances of every structure type from/to another type is also calculated and illustrated in Fig.~\ref{fig:Imshow}. It is vividly clear that the isolated atom and the dimer configurations have a huge distance from almost everything. However, they are kept in the dataset due to the fact that DFT calculations for such small cells are rather cheap and they will not affect the Neural Network so much. The same story is true for simple cubic, A15, C15 and diamond configurations. On the other hand, liquid configurations are deleted from the dataset since they are computationally expensive, and based on the distribution of their distances from the indented configuration shown in Fig.~\ref{fig:Liquid_Dis}.a the population of the atoms is the most around the threshold distance. Also, only half of the self-interestitials (SIA) are kept in the dataset. The reason is due to the fact that, not only the distribution of their distances from the indented configuration has a big tail, but it is also believed that the pick of the distribution around small distances comes from the bulk region of the SIA supercells, Fig.~\ref{fig:Liquid_Dis}.b.


\subsection{DFT calculations}

The DFT calculations were performed with the \texttt{Quantum Espresso} \cite{Giannozzi_2009, Giannozzi_2017} (QE) package, using a norm-conserving PBEsol exchange-correlation functional \cite{Prandini2018, doi:10.1126/science.aad3000, PhysRevB.88.085117} and 14 valence electrons. The Brillouin zone was sampled using Monkhorst-Pack method \cite{PhysRevB.13.5188}, and, from the convergence analysis of Fig.SM-2, the k-point mesh and plane-wave cutoff energy in a Mo unit-cell were set to $8\times8\times8$ and 60 $Ry$, respectively. The selected k-point grid was rescaled for supercells calculations according to their dimension, implying the use of a $2\times2\times2$ grid for $4\times4\times4$ conventional super-cells, and was set to $1\times1\times1$ for any bigger configuration. Smearing was introduced within the Methfessel-Paxton method \cite{PhysRevB.40.3616} to help convergence, with a spreading of 0.00735 $Ry$ (0.1 $eV$). The structural properties, involving elastic constants $C_{ij}$, Bulk modulus $B$ (in the Voigt-Reuss-Hill approximation~\cite{chung1967voigt}) and Poisson ratio $\nu$, have been computed running the QE driver \texttt{THERMO\_PW}~\cite{thermopw} on a Mo unit-cell.

The total energies of the configurations obtained from~\cite{dataset} were compared with the values calculated in our work to make sure of their consistency, which is shown in Fig.SM-4. 

\subsection{Neural Network Training}

In the PANNA framework, the environmental descriptors of each atom are provided as input to a fully connected network with two hidden layers, consisting of 256 and 128 nodes for the first and second layers, respectively, both with Gaussian activation function, and a single-node output layer with linear activation. The atomic environment is represented by a descriptor with 152 components, resulting in a network with 71808 weights and 385 biases.
%(152 × 256 + 256 × 128 + 128 × 1 = 71808; 256+128+1 = 385). 
A batch size of $10$ 
is utilized for training, while the model is trained using initial random weights and a constant learning rate of $10^{-4}$ throughout the training process. In this methodology, the energy of a configuration consisting of $N$ atoms is defined as the sum of atomic energy contributions:
\begin{equation}\label{energy}
E = \sum_{i=1}^NE_i(G_i),
\end{equation}
where $E_i$ is the energy of atom $i$ with a G-vector of $G_i$. 
The force on atom $i$ 
which is situated 
at position $\vec{R}_i$
is given by:
\begin{equation}\label{force}
\vec{F}_i = -\sum_{j}\sum_{\mu}\frac{\partial E_j}{\partial G_{j\mu}}\frac{\partial G_{j\mu}}{\partial \vec{R}_i}
\end{equation}
with $j$ labeling the atoms located within the cutoff distance of atom $i$
and $\mu$ labeling the descriptor components. 

To optimize the weights and bias parameters of the network, we use the Adam algorithm~\cite{kingma2017adam} 
to compute gradients of randomly selected batches of the training dataset. 
The loss function for optimizing the network weights, 
denoted collectively as $W$, consists of 
two terms, one for 
the energy $\mathcal{L}_E(W)$, 
and one for the forces, 
$\mathcal{L}_F(W)$:
\begin{equation}\label{losstotal}
    \mathcal{L}(W) = \mathcal{L}_E(W) + 
    \mathcal{L}_F(W).
\end{equation}
%\begin{equation}
%    \begin{aligned}
%    \mathcal{L}_E(W) &= \sum_{c \in batch} \left( E_{(c)}^{DFT} - E_c(W) \right)^2 \\
%    &\quad + \exp \left[ \operatorname{atanh} \left( \frac{1}{a} \sum_{c \in batch} %\left( \frac{E_{(c)}^{DFT} - E_c(W)}{N_c} \right)^2 \right) \right] \\
%    \end{aligned}
%\end{equation}
The energy contribution is given by:
\begin{equation}\label{lossenergy}
%    \begin{aligned}
    \mathcal{L}_E(W) = \sum_{s \in {\rm batch}} \left[ E_{s}^{{\rm DFT}} - E_{s}(W) \right]^2 
    % \\
 %   &\quad
%    \end{aligned}
\end{equation}
where $s$ refers to 
the atomic configuration, 
$E_{s}^{DFT}$ 
is the total energy calculated from DFT (the target value) 
and $E_s(W)$ is the total energy predicted by the NNIP. 
The force contribution is given by:
\begin{equation}\label{lossforce}
    \mathcal{L}_F(W) = \lambda_F \sum_{s \in {\rm batch}} \sum_{i=1}^{N_s} \left\lvert \vec{F}_{i;s}^{{\rm DFT}} - \vec{F}_{i;s}(W) \right\rvert^2
\end{equation}
with $\vec{F}_{i;s}^{{\rm DFT}}$ the force obtained from DFT 
and $\vec{F}_{i;s}$ 
the force obtained from the NNIP, 
for atom $i$ in configuration $s$; 
$N_s$ is the total number of atoms in configuration $s$. 
The parameter $\lambda_F$  
adjusts the 
relative contribution of the force component 
and was set to 
$\lambda_F =0.5$. 

%####### Nanoindentation
\subsection{Nanoindetation simulations}

\subsubsection{Simulation method and parameters}
To establish boundary conditions along the depth ($dz$) of the Mo samples, we 
divided them into three sections in the $z$ direction during the initial stage: 
a frozen section with a width of approximately 
0.02$\times dz$, which ensured numerical cell stability; a thermostatic section 
about 0.08$\times dz$ above the frozen section, which dissipated heat generated 
during nanoindentation; and a dynamical atoms section, where the interaction with 
the indenter tip modified the surface structure of the samples. 
Furthermore, we 
included a 5 nm vacuum section at the top of the sample as an open boundary 
\cite{KURPASKA2022110639}.
We considered the indenter tip as a non-atomic repulsive imaginary (RI) rigid 
sphere and defined its force potential as 
\begin{equation} 
F(t) = K \left(\vec r(t) - R 
\right)^2,
\end{equation} 
where $K = 236$ eV/\AA$^3$ (37.8 GPa) was the force constant, and 
$\vec r(t)$ was the position of the center of the tip as a function of time, with 
a radius $R = 3$ nm. We conducted molecular dynamics (MD) simulations using an 
NVE statistical thermodynamic ensemble and the velocity Verlet algorithm to 
emulate an experimental nanoindentation test. The $x$ and $y$ axes had periodic 
boundary conditions to simulate an infinite surface, while the $z$ orientation 
had a fixed bottom boundary and a free top boundary in all MD simulations 
\cite{DOMINGUEZGUTIERREZ2021141912, PhysRevMaterials.7.043603}.

In our simulations, we chose $\vec r(t) = x_0 \hat x + y_0 \hat y + 
(z_0 \pm vt)\hat z$, where $x_0$ and $y_0$ were the center of the surface 
sample on the $xy$ plane, and $z_0 = 0.5$ nm was the initial gap between 
the surface and the indenter tip. The tip moved with a speed of 
$v = 20$ m/s with a 
time step of $\Delta t = 1$ fs. We chose the maximum indentation depth 
to be 2.0 nm to avoid the influence of boundary layers in the dynamical
atoms region.

\subsubsection{Normalized maximum shear stress}

The contact pressure, $P$, is calculated by using a linear elastic
contact mechanics formulation 
\cite{PhysRevMaterials.7.043603,VARILLAS2017431}:
\begin{equation}
    P = 2\pi  
    \left[ 24p \left( \frac{E_{\rm Y}R}{1-\nu^2} \right)^2 \right]^{1/3},
    \label{eq:pressure}
\end{equation}
with $E_Y$ as the Young's modulus, $p$ as the simulation load, $R$
the indenter radius, and $\nu$ the Poisson's ratio;
the radius of the contact area is obtained with the geometrical 
relationship: 
\begin{equation}
\mathrm{a}(h) = \left[ 3PR \left( 
 1-\nu^2\right)/8E_{\rm Y} \right]^{1/3}
 \end{equation}
 which is related to the  inner radius 
 of the plastic region where the defects nucleate.
 This quantity provides an intrinsic measure of the surface resistance 
 to a specific defect nucleation 
 process~\cite{VARILLAS2017431,PhysRevMaterials.7.043603}.
To determine the strength and stability of the Mo
matrix under load, 
we compute 
the principal stress applied on the $z$ direction
as \cite{REMINGTON2014378} :
\begin{equation}
%\resizebox{\columnwidth}{!}{%
    \sigma_{zz}  = 
    %& 
    - \mathcal{S}
    %\left( \frac{3F}{2 \pi \mathrm{a}(h)^2}\right) 
%    \nonumber \\
%    & 
    \left[ \left( 1-
%    \left|\frac{z}{\mathrm{a}(h)} \right| 
\frac{
    \arctan 
    (\alpha)}
    {\alpha}
%    \left|\frac{\mathrm{a}(h)}{z} \right| 
    \right) 
    (1+\nu)
   -\frac{1}{2(1+
   1/\alpha^2)
%   z^2/\mathrm{a}(h)^2)
   }  \right],   
   %}
\end{equation}
where the quantities 
$\mathcal{S}$ and $\alpha$ are defined as:
\begin{equation}
    \mathcal{S} =
    \frac{3P_{\rm ave}}{2 \pi \mathrm{a}(h)^2},
    \quad
%\end{equation}
%and
%\begin{equation}
    \alpha = 
    \frac{\mathrm{a}(h)}{h}.
    \nonumber
\end{equation}
with $h$ as the indentation depth and $a(h)$ the contact area between 
the indenter tip and the top atomic layers.
%\textcolor{blue}{
%NOTE: you must define the meaning of the variables $\mathrm{a}(h)$
%that appear in the above equations.
%}\\
The stress applied in the direction parallel to the indenter 
surface is then expressed as:
\begin{equation}
    \sigma_{xx}  =  \sigma_{yy} = - %\left( \frac{3F}{2 \pi \mathrm{a}(h)^2}\right) 
\frac{\mathcal{S}}{1+1/\alpha^2
%z^2/\mathrm{a}(h)^2
}
\end{equation}
%where $x,y$, and $z$ are the coordinates in the Cartesian system.  
This gives the maximum shear stress: 
\begin{equation}
\tau_{\rm max} =
\frac{1}{2} 
\left( \sigma_{zz}-\sigma_{xx} \right),
\label{eq:shearMax}
\end{equation}
that the material can withstand 
before it begins to undergo plastic deformation, being normalized by the applied pressure (equal to the applied 
force
$F$ divided by the contact area). 
The normalized depth is the distance from the surface of the material to the 
point at which the maximum shear stress occurs, 
normalized by the radius of the indenter that is used 
to apply the shear forces. 

\subsubsection{Defect analysis}

In order to identify the defects in nanoindentation 
simulations, we apply the BCC Defect Analysis (BDA) 
developed by M\"oller and Biztek~\cite{moller2016bda} 
which utilizes coordination number (CN), centrosymmetry 
parameter (CSP), and common neighbor analysis (CNA) 
techniques to detect typical defects found in
bcc crystals. 
The characterization of the materials defects starts 
by calculating CN, CSP, and CNA values of all the atoms by 
considering a cutoff radius of $(1+\sqrt{2})/2a_0$ with $a_0$ 
as the lattice constant of Mo.
Thus, the six next--nearest neighbors of perfect bcc atoms
are into this cutoff and their CN value increases from 8 to 14. 
Consequently, BDA compares the CN and CSP values of each atom 
generating a list of non--bcc neighbors with 
CNA$\neq$bcc and CN$\neq$14 that classifies for the following 
typical defects: surfaces, vacancies, twin boundaries, screw 
dislocations, \{110\} planar faults, and edge dislocations.

==> sections/Results.tex <==
\section{\label{sec:Results}Results}

\subsection{Dataset evaluation and improvement}


%%%%%%%%%%% Table 1
\begin{table}[b!]
\centering
\caption{The original dataset from~\cite{dataset}. showing $N_s$ as the number of structures, $N_{at}$ as the number of atoms per configuration, and $N_{sel}$ as the number of selected configurations in the final dataset.}
\label{tab:tabale1}
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{crrr}
\hline
Structure type & $N_s$	& \; \; $N_{at}$    & \; \; $N_{sel}$\\
\hline
Isolated atom		  & 1     & 1      & None\\
Dimer           	  & 19    & 2      & None\\
Slice sample		  & 1996  & 1      & All\\
Distorted BCC         & 547   & 2      & All\\
A15                   & 100   & 8      & None\\
C15                   & 100   & 6      & None\\
HCP                   & 100   & 2      & All\\
FCC                   & 100   & 1      & None\\
Diamond               & 100   & 2      & None\\
Phonon                & 50    & 54     & All\\
Self-interstitials (SIA)    & 32    & 121    & 14\\
di-Self-interstitials & 14    & 122-252& All\\
Simple Cubic          & 100   & 1      & None\\
Vacancy               & 210   & 53     & All\\
di-Vacancy            & 10    & 118    & All\\
tri-Vacancy           & 14    & 117    & All\\
Liquid                & 45    & 128    & None\\
Short range           & 90    & 53-55  & None\\
Surface (100)         & 45    & 12     & All\\
Surface (110)         & 45    & 12     & All\\
Surface (111)         & 41    & 12     & All\\
Surface (112)         & 45    & 12     & All\\
Liquid Surface        & 24    & 128    & All\\
$\gamma$-urface         & 178   & 12     & All\\
\textbf{GSFCs}        & 100   & 18     & All \\
\textbf{GSFCs + SIA}  & 100   & 55     & All \\
\textbf{Pileup}       & 1000  & 32     & All \\
\textbf{HT + substrate} & 600 & 54-72  & All \\

\hline
\end{tabular}
}
\end{table}



\begin{figure*}[t]
  \centering
  \includegraphics[width=0.98\textwidth]{Figs/fig1.png}
  \caption{Dataset evaluation and stability. a)Average of minimum distances between different configuration types as well as with the indented samples. b) Distribution of the minimum distances of different configurations in the dataset and the minimum distances of the dataset with the indented configurations. c) Effect of configuration removal from the dataset on minimum distances of the dataset to the indented sample.} 
  \label{fig:originaldataset}
\end{figure*} 

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.98\textwidth]{Figs/Fig2.png}
  \caption{Illustration of the novel configurations discovered in this study, which correspond to distinct regions of an indented sample. The figures are arranged horizontally to demonstrate the correlation between them. a) The distances of the dislocation cores, atoms beneath the indenter tip, and pileup atoms on the surface from the original dataset. b) The newly detected high-temperature configurations, which are associated with diverse regions of the indented sample, in terms of their distance. c) The distance of the aforementioned regions shown in panel (a) after incorporating the newly found configurations to the dataset. d) The distribution of distances of the aforementioned atoms from the dataset before and after incorporating the newly introduced configurations.} 
  \label{fig:newconfigs}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.98\textwidth]{Figs/fig33.png}
  \caption{The impact of incorporating Generalized Stacking Fault Configurations (GSFCs) on the distances of atoms on dislocation cores from the dataset. a) A schematic representation of the GSFCs integrated into the dataset. b) Addition of GSFCs reduces the distances of atoms on the slip plane of dislocation cores from the dataset. c) By including an SIA on the surface of GSFCs, all atoms on the dislocation cores can be covered. d) The distribution of atom distances on dislocation cores reveals that GSFCs with SIA can effectively cover dislocation cores.} 
  \label{fig:GSFCs}
\end{figure*}


As a starting point, we used a dataset~\cite{dataset} originally developed to train a ML potential within the GAP framework~\cite{PhysRevLett.104.136403,PhysRevMaterials.4.093802}. The objective was to 
determine whether this dataset accurately represents the atomic configurations 
occurring during nanoindentation simulations, for which we
employed an EAM potential~\cite{ESalonen_2003}. 
We then analyzed the 
obtained data to determine the degree of similarity between the atomic 
configurations in the dataset and those observed during the indentation 
simulations.
This level of similarity is evaluated by identifying which atom $j$ in the dataset has the minimum distance to each atom $i$ in the indented sample. The obtained value corresponds to the \emph{largest minimum} distance for each atom in the indented sample from all the atoms in the dataset. The concept of ``distance'' for two atoms $i$ and $j$, refers to the $l^{2}$-norm of $G_{i}[s] - G_{j}[s]$, where $G[s]$ are the fixed-size modified Behler-Parinnelo (mBP) descriptor vectors~\cite{C6SC05720A, PhysRevLett.98.146401} used in this work (see \textbf{Methods and Materials} for more details).
To this end, we compared the configuration 
types present in the dataset to those of all atoms identified in the indented 
sample and drew conclusions based on the level of correspondence between the two sets. 
Through this analysis, we aimed to gain insights into the suitability of the 
selected dataset for studying nanoindentation behavior and identifying the 
underlying mechanisms governing it.

To create an appropriate dataset to train an interatomic potential aimed at nanoindentation simulation, it is crucial to ensure that the configurations included accurately represent the three essential regions of a sample under indentation. These regions include the atoms on the surface of the sample, which correspond to the pileup patterns, the atoms situated beneath the indenter tip that undergo significant plastic deformation, and the atoms located on the nucleated dislocation cores. The 
evaluation of these three critical regions and 
development of configurations that closely resemble them can 
serve as a 
benchmark
for ML potentials for other BCC materials.

Before comparing the original dataset with the indented sample, we calculated the average minimum distance between each pair of configuration types and generated a correlation figure to visualize their proximity (Figure ~\ref{fig:originaldataset}-a).  
It is evident from this figure that although the isolated atom and dimer configurations are quite distant from almost all other configurations, they are relatively close to the indented samples. However, these configurations were not included in the final dataset due to their low numbers (1 and 19, respectively), which were deemed insufficient for training a NNIP. Moreover, the A15, simple cubic (sc), diamond (dia), liquid and C15 configurations were removed from the final dataset as they were located at a distance of 6 ~ (the chosen threshold will be discussed later) or more from the indented configurations, with simple cubic, diamond, and C15 configurations having the largest distance. Furthermore, we excluded short-range configurations from the final dataset because their energies varied significantly (Figure SM.1-a), leading to training difficulties. Finally, to reduce computational cost, we kept only half of the self-interstitial configurations in the final dataset. Table ~\ref{tab:tabale1} summarizes all modifications made to the original dataset.

Several methods can be employed to determine a ``good" threshold for deciding whether to keep or remove a particular configuration from the dataset, based on its similarity to the intended configuration. In this study, we have chosen to use the start of the tail of the distribution of the minimum values in the dataset's distance matrix as the threshold, which is approximately 6 based on Figure.~\ref{fig:originaldataset}-b. Figure.~\ref{fig:originaldataset}-b also demonstrates that this value is consistent with the minimum distances between the dataset configurations and all three orientations of the indented samples. All decisions regarding whether to keep or remove a configuration from the final dataset in this study are based on this threshold.

To ensure the accuracy of the modifications made to the dataset, we removed one type of configuration from the dataset at a time and quantified the number of atoms in the intended samples that had minimum distances greater than 5 from the dataset (Figure.~\ref{fig:originaldataset}-c). As our analysis shows, the number of atoms with a minimum distance greater than 5 to the dataset does not increase when A15, diamond, Face-Centered Cubic (FCC), simple cubic, short range, isolated atom, and dimer configurations are removed, indicating the dataset's stability against the indented samples, whether these configurations are present in the dataset or not. However, upon removing Hexagonal Close-Packed (HCP) configurations, the number of atoms with a large distance from the dataset increases, which is consistent with the fact that the average minimum distance of HCP configurations to the intended samples is 5 . The greatest increase in the number of atoms with a distance greater than 5 ~ from the dataset occurs when surface configurations are removed, which underscores their importance since they represent the surface in the nanoindentation simulations.

Following the modifications made to the dataset obtained from \cite{dataset}, attempts were made to enhance its quality by incorporating various types of configurations and reevaluating the distances of the indented configuration from the dataset. Among the crucial local environments that should be included in the dataset are the atoms belonging to the dislocation cores. Furthermore, it was discovered that the distances of the atoms beneath the indenter tip and those on the surface exceeded the selected 6 threshold (Figure.~\ref{fig:newconfigs}-a). These environments in the indented samples are critical to be covered in the dataset since dislocation cores play a vital role in the dislocation dynamics properties, and the atoms beneath the indenter tip trigger these line defects. Additionally, the plastic region beneath the surface is responsible for the pile-up patterns that appear on the surface of the indented configuration. It is also imperative to incorporate configurations in the dataset representing atoms on the surface to capture this phenomenon.

In order to model the aforementioned regions of an indented sample, we explored the use of high-temperature configurations to effectively reduce the distance between the atoms in these areas and the dataset, as depicted in Figure.~\ref{fig:newconfigs}-b. Nevertheless, accounting for the atoms beneath the indenter tip and on the surface requires the inclusion of a layer of frozen atoms in the high-temperature configurations that emulate the contact of the sample with the indenter tip. The addition of $1000$ isothermal-isobaric ensemble (NPT) high-temperature configurations with $16$ atoms in the $2 \times 2 \times 2$ supercells appeared to decrease the distances between the atoms on the dislocation cores and the dataset. We utilized the same approach for the atoms beneath the indenter tip. In this regard, we introduced $600$ configurations, denoted as ``high temperature $+$ substrate", where a layer of atoms was frozen while other atoms were heated to high temperatures (under the melting point). While there are various unique layers of atoms that can be taken into account as the contact to the substrate, we verified that 300 configurations ($3 \times 3 \times 3$) with $54$ atoms per supercell---displayed in the middle figure of Figure.~\ref{fig:newconfigs}-b---were adequate and most relevant after trying different layers of atoms. Additionally, we included 300 configurations ($4 \times 3 \times 3$) with $72$ atoms per supercell, which featured a layer of atoms frozen on top. Moreover, it is crucial for a NNIP's dataset to incorporate configurations resembling the atoms located on the surface of the indented sample. To achieve this, we introduced $1000$ BCC surface configurations ($3 \times 3 \times 2$) with $32$ atoms per supercell, where a layer of atoms was frozen on top while the remaining atoms were subjected to high temperature. These configurations were named ``pileup" in our study and enabled the dataset to account for the atoms in this region.

Another effective approach to cover the dislocation cores is through the use of Generalized Stacking Fault Configurations (GSFCs) that incorporate a self-interstitial atom (SIA) atom on the surface (as illustrated in Fig.3a). These configurations have been found to be particularly effective in reducing the distances of atoms on the dislocation cores from the dataset. While the use of GSFCs without an SIA on the surface can also reduce distances of atoms beneath the dislocation cores and on the slipping plane (as shown in Figure \ref{fig:GSFCs}-b), it may not entirely cover all the atoms on the dislocation core.

Incorporating an SIA on the surface of the GSFCs leads to a significant decrease in the distances of almost all atoms on the dislocation cores from the dataset (as demonstrated in Figure \ref{fig:GSFCs}-c). Notably, the use of GSFCs with SIA configurations instead of high-temperature configurations solely for the dislocation cores presents several advantages. For instance, the distribution of energies of these configurations is narrower, facilitating the learning process for the network (as depicted in Figure SM.1-b). Furthermore, only $100$ GSFCs with SIA configurations, as opposed to the $1000$ mentioned for high-temperature configurations, can ease the process of training
the network. Additionally, using GSFCs with SIA configurations guarantees that no atoms on the dislocation core will have a distance greater than 6, thus ensuring the closeness of the distances of these configurations to the dislocation cores.

The visualization of the distances between the atoms in all three regions of interest and the dataset reveals a significant reduction in distances after incorporating the high-temperature configurations (see Figure.~\ref{fig:newconfigs}.c). The distribution of distances for each region before and after adding the high-temperature configurations is depicted in Figure.~\ref{fig:newconfigs}.d. 
Although a few atoms still have distances greater than  6 under the indenter tip, the number of such atoms has notably decreased after adding the appropriate configurations. Finally, because we are trying to develop  a NNIP for the case of nanoindentation simulation during which atoms are compressed under the indenter tip, we added $300$ compressed $3 \times 3 \times 4$ configurations with each of them including 72 atoms.

\subsection{NNIP predictions 
%on the Energies and Forces
}

We assessed the accuracy of the trained NNIP by calculating the root mean square error (RMSE) for both energies per atom (E-RMSE) and forces components (F-RMSE) at each checkpoint saved during training. To ensure the reliability of the final model on unseen data, $10 \%$ of configurations of each structure type were reserved for validation prior to training. Fig. \ref{fig:val} shows that both the F-RMSE and E-RMSE decrease gradually as the network processes more data, reaching a plateau after 850K training steps with minimum values of 9.2 meV/atom and 0.16 eV/\AA, respectively.

%In this work, a configuration type based error validation is taken into account. For the validation purposes, 10 percent of configurations of each structure type is kept before training, to make sure of the performance of the final model on the data unseen by the network. The root mean square error (RMSE) for both total energies (E-RMSE) and forces (F-RMSE) is calculated and reported in Table.(~\ref{T_3}). Since the efficiency of the model on the configurations that matters most in nanoindentation simulations is of high importance, only "high temperature", "fixed layer", "upper layer fixed", "compressed" and "pileup" structures are considered in the validation study. The E-RMSE values are all less than 10 meV/atom and the F-RMSE values are maximum 413 mev/\AA. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.47\textwidth]{Figs/validation_2.png}
  \caption{Prediction of the Energies and forces for the validation set during the NNIP training.} 
  \label{fig:val}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.48\textwidth]{Figs/fig4.png}
  \caption{NNIP error on \textbf{(a)} total energies and \textbf{(b)} forces of each atom.} 
  \label{fig:EVal}
\end{figure}


%%%%%%%%%%%% Table 2
%\begin{table}[b!]
%\centering
%\caption{caption}
%\label{tab:tabale2}
%\resizebox{0.75\columnwidth}{!}{%
%\begin{tabular}{crrr}
%\hline
%Configuration type & $E-RMSE$	& $F-RMSE$    &\\
%\hline
%GSFCs                        &  float & float \\
%GSFCs + SIA                  &  float & float \\
%Pileup                       &  float & float \\
%HT + substrate               &  float & float \\
%Validation set               &  float & float \\

%\hline
%\end{tabular}
%}
%\end{table}
%%%%%%%%%%%%% table2


The error distribution for both energies and forces follows closely a Gaussian distribution, as shown in the histogram plot of Fig.\ref{fig:EVal}(a,b). The two islands in Fig. \ref{fig:EVal}(a) are due to the energy difference between the pure and defected crystals. Also, the presence of three clusters in Fig. \ref{fig:EVal}(b) is due to the large forces on the atoms in the defected configurations. 

%The energy validation of the above mentioned configurations are also illustrated in Fig.~\ref{fig:parity}. It is clear that the final model is functioning greatly on the energy prediction. Furthermore, the energy and force prediction on the validation set is shown throughout the training in Fig.~\ref{fig:val}. The plateau at the end of the plots shows that the local minima is found and the training could be stopped after 700000 training steps.

%\subsection{NNIP prediction on elastic constants}

%In this section, 
Next, we compare 
the elastic properties of the NNIP interatomic potential 
with both DFT and experimental results, 
as well as to 
those predicted by other interatomic potentials, such as GAP, tabGAP, and the EAM/FS potential,
to evaluate the NNIP
performance relative to other commonly used potentials.
Table \ref{tab:elastic} shows the results of the comparison, and it can be seen that the NNIP performs well for most of the elastic properties studied, with errors not exceeding $5\%$ compared to both DFT and experiment. The largest error for the NNIP is about $23\%$ for the $C_{12}$, which is still within a reasonable range considering the complexity of the system being studied. The other potentials also have good predictions for most of the elastic properties, except for tabGAP, with a comparatively higher error of $22\%$ for the $C_{44}$.

The importance of accurately predicting the shear modulus, $C_{44}$, is highlighted, as it is crucial for nanoindentation simulations. Accurate prediction of the shear modulus is
essential for simulating the stresses that are applied to the surface of the sample during this process. The NNIP predicts the $C_{44}$ value very well, with an error of only $5\%$, making it a promising interatomic potential for nanoindentation simulations.

%%%%%%%%%%% Table 3
\begin{table}[b!]
\centering
\caption{Elastic
constants $C_{ij}$, bulk modulus $B$, and Poisson ratio $\nu$, 
as obtained with the GAP, tabGAP, EAM/FS and the NNIP potentials compared to DFT done in this work and experimental data from \cite{rumble2019crc}.}
\label{tab:elastic}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{crrrrrr}
\hline
 & GAP & tabGap & EAM & NNIP	& DFT & Exp\\
\hline
$C_{11}$ (GPa) & 478 & 494 & 465 & 452 & 459 & 464\\
$C_{12}$ (GPa) & 166 & 146 & 161 &  121 & 162 & 159\\
$C_{44}$ (GPa) & 108 & 87 & 109 &  111 & 97 & 109\\
%\hline
$B$ (GPa) & 270 & 262 & 263 &  231 & 262 & 250\\
$\nu$ & 0.26 & 0.23 & 0.26 &  0.21 & 0.30 & 0.29\\
\hline
\end{tabular}
}
\end{table}
%%%%%%%%%%%%% table 3



%\subsection{NNIP prediction on the interstitial and vacancy formation energies}

%%%%%%%%%%% Table 2
%\begin{table}[h!]
%\centering
%\caption{Point defect formation energy}
%\label{tab:tabale2}
%\resizebox{0.95\columnwidth}{!}{%
%\begin{tabular}{crrrrrr}
%\hline
%$E_{f}$ & tabGAP & EAM & GAP & NNIP	& DFT\\
%\hline
%$\langle111\rangle$ & 8.05 & 6.68 & 8.29 & 8.44 & 7.14\\
%$\langle110\rangle$ & 7.75 & 6.44 & 8.29 &  8.65 & 7.17\\
%$\langle100\rangle$ & 8.92 & 6.68 & 9.67 &  9.41 & 8.53\\
%Octa & 8.83 & 6.38 & 9.65 &  9.82 & 8.59\\
%Tetra & 8.68 & 6.42 & 9.16 &  8.65 & 8.04\\
%Vac & 3.12 & 2.58 & 3.03 & 2.84 & 3.35\\

%\hline

%\end{tabular}
%}
%\end{table}
%%%%%%%%%%%%% table2

%\subsection{NNIP prediction on generalized stacking fault energy}

%This section discusses the comparison of the 
Finally, we compare the 
NNIP predictions for the GSFE against the DFT results, as well as other interatomic potentials mentioned in this work. The study focuses on the two most important slip systems of BCC crystals, namely the $\{110\}\langle\bar111\rangle$ and $\{121\}\langle\bar111\rangle$ families. The results were obtained for these directions in pure crystals. Additionally, since it was observed from Fig. \ref{fig:GSFCs} that GSF $\{110\}\langle111\rangle$ configurations with a $\langle111\rangle$ dumbbell interstitial on the surface cover the atomic environments of the dislocation core in terms of their distance to the indented samples, we also calculated and compared the GSFE for these configurations. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.48\textwidth]{Figs/Mo_GSFE.png}
  \caption{Generalized Stacking Fault Energy (GSFE) for single crystalline Molybdenum for: (a) $\{110\}\langle\bar111\rangle$ and (b) $\{211\}\langle\bar111\rangle$. 
  (c) The GSFE curve for the "GSFCs $+$ SIA" configurations.} 
  \label{fig:GSFE}
\end{figure}

Fig. \ref{fig:GSFE} shows that all potentials except for EAM/FS predict the GSFE very accurately for both slip system families and pure crystals. However, EAM/FS has errors of about $50\%$ and $32\%$ for the peak of the curve for $\{110\}\langle\bar111\rangle$ and $\{121\}\langle\bar111\rangle$ slip families, respectively. The configurations associated with these curves are crucial, as they represent the atoms on the slip plane of an indented sample, as illustrated and discussed in 
Fig. \ref{fig:GSFCs}. 
While it is important for an interatomic potential to accurately predict the GSFE curve for reliable dislocation modeling, it is equally crucial for the potential to correctly predict the energies and forces on the atoms for 
the dislocation cores. Therefore, in addition to the GSFE curves for pure crystals, we calculated the GSFE curve for configurations with a $\langle111\rangle$ dumbbell interstitial on the surface. As depicted in Fig. \ref{fig:GSFE}(c), NNIP is the potential that best predicts these energies, indicating the accurate simulation of dislocation dynamics during nanoindentation. In contrast, GAP and EAM potentials showed errors of $40\%$ and tabGAP showed an error of $20\%$ against DFT results, indicating their inability to accurately predict these values. This is discussed further in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{NNIP Nanoindentation}

\begin{figure} 
    \centering
    \includegraphics[width=0.48\textwidth]{Figs/FigMaxShear.png}
    \caption{Hertzian calculation of normalized maximum shear
    stress by the applied pressure, $\tau_{\rm max}/P$, as 
    a function of normalized depth for main crystal orientations. 
    Surface information is needed in the interatomic potentials to 
    model nanoindentation induced plasticity in the 
    range of 0.0 to 0.475 $d/a$.
    To aid the  interpretation of the results, the values for EAM/FS were shifted by $-0.1$, the values for GAP were shifted by $+0.2$, and the values for tabGAP were shifted by $+0.1$ (all values in units of $\tau_{\rm max}/P$). 
    %These shifts were applied to the data to improve the clarity and distinguishability of the plotted results.
    %\textcolor{blue}{NOTE: The label on the vertical axis should be $\tau_{\rm max}/P$.
    %The label on the horizontal axis should be: Indenter-tip displacement ($d/a$).}
    }
    \label{fig:maxstress}
\end{figure}
Plastic deformation 
does not initiate at the surface, 
but rather at a certain depth below it, 
typically a few atomic layers deep. 
This depth is known as the ``yield point'' or ``yield depth'', at which point the 
material begins to nucleate defects and dislocations under the 
applied load or stress. %\textcolor{blue}{which is calculated 
%by Eq. \ref{eq:shearMax}. 
The initiation of the plastic deformation of the material 
occurs within the closest plastic region along the 
vertical $z$-axis beneath the spherical indenter tip.
In Fig.~\ref{fig:maxstress} we show results for the 
normalized maximum shear stress $\tau_{\rm max}/P$ %\textcolor{blue}{
%by using Eq. \ref{eq:shearMax}}
which is a dimensionless quantity, with $P$ being
the applied pressure (Eq. 
\ref{eq:pressure}) and  $\tau_{\rm max}$ the shear stress (Eq. \ref{eq:shearMax}) calculated by using a linear elastic
contact mechanics formulation 
\cite{PhysRevMaterials.7.043603,VARILLAS2017431},
as a function of the displacement $d$ for [001], [011], and [111] 
main crystal orientations~\cite{PhysRevMaterials.7.043603}. A detailed explanation of the normalized shear stress calculation is provided in the \textbf{Methods} section. 

Our MD simulations report enough surface energy to model 
the nanoindentation induced plasticity as observed at distances 
close to the sample surface regardless of the crystal orientation, 
which is 
challenging for traditional and current ML
interatomic potentials for BCC Mo.
The modeling of the nanocontact of the indenter tip 
and the top atomic layers of the surface, from 0 to $\sim 0.3$ $d/a$ range with $d$ 
the indentation depth and $a$ the contact area, 
is important due to the nucleation of dislocation is dependent
on this mechanisms.\\
%\textcolor{blue}{NOTE: The quantities $a$ and $d$ have not been defined.}\\

The GAP simulations provide valuable insights into the interaction
between the indenter tip and the top layer atoms for the (001) and (011) orientations.
However, for the (111) orientation, this information is lacking, resulting in a 
limitation in accurately modeling the nanoindentation test before the yield point.
This limitation arises due to the absence of the relevant atomic configurations in the training data for this
specific potential.
As a consequence, the tabGAP simulations follow a similar trend for the (111)
orientation, reflecting the lack of detailed information on the interaction between
the tip and the surface atoms.

In contrast, the NNIP simulations incorporate sufficient  information on
surface structures, allowing for a more accurate representation of the contact area. 
This is particularly important as the contact area depends on the applied load. 
The computed force between the tip and the atoms comprising the contact area is well-modeled in the NNIP simulations. 
The difference in spacing between data points in the elastic part of the graph is attributed to variations in the loading force, pressure, and maximum shear stress, which are considered in the contact area analysis.

Fig.~\ref{fig:bda_method} illustrates the defects detected 
using the BCC Defect Analysis (BDA)
method (see \textbf{Methods}) in a (111) Mo sample at different depths \cite{moller2016bda}. 
%The representation of material defects is as follows: gray spheres represent surface atoms in direct contact with the indenter tip, blue spheres represent edge dislocations, light-blue spheres depict atoms near vacancies, yellow spheres denote twin/screw dislocations, and black spheres indicate unidentified defect atoms. 
The NNIP nanoindentation simulations in
the initial stages of loading process notably enhance 
the description of the interaction between the indenter tip
and the atoms in the uppermost layers of the surface (see Fig. 
\ref{fig:bda_method}a). 
In this context, a few Mo atoms located at the very top 
surface layer are recognized as surface defects. 
Additionally, Mo atoms situated beneath these surface defects
begin to coalesce, forming edge dislocations that have 
the potential to evolve into shear loops. 
Contrary to the other simulations where the interatomic 
potentials are not aware of this mechanism.
NNIP simulations are also
anticipated to accurately capture the nucleation and 
propagation of shear loops on \{112\} planes (See Fig. 
\ref{fig:bda_method}b), as observed experimentally in BCC 
materials \cite{VARILLAS2017431,REMINGTON2014378,MULEWSKA2023154690}. 
Furthermore, NNIP effectively models the nucleation of 
loops through a lasso mechanism, a behavior where GAP and tabGAP 
induced the formation of multiple loops, 
as observed in Fig \ref{fig:bda_method}c) at a depth of 1.45nm. 
For NNIP, at the maximum indentation depth, it is evident on the sample's surface that displaced atoms align with the slip planes in a 
characteristic three--folded rosette pattern typical for BCC 
materials in the [111] orientation (Fig \ref{fig:bda_method}d), 
formed by [11$\Bar{2}$], [$\Bar{1}$01], and [0$\Bar{1}$1] 
planes.
In contrast, 
neither GAP nor tabGAP, nor EAM, can adequately incorporate
this description due to the lack of information regarding
pile--up formations.
Besides, the nucleation of more loops is noted, but the 
circumference of the second loop is larger than that of
the first loop. 
The EAM and tabGAP simulations demonstrate a slower and faster 
process, respectively.



\begin{figure}[t!]
    \centering
    \includegraphics[width=0.48\textwidth]{Figs/bda_all.png}
    \caption{
    %(Color online) 
    Identified defects of indented 
    (111) Mo sample by BDA method at different depths by NNIP, 
    EAM, TabGAP, and GAP approaches. 
    The various defect types are 
    depicted using different colors: gray spheres represent 
    surface atoms in direct contact with the indenter tip, blue 
    spheres indicate edge dislocations, light-blue spheres 
    represent atoms in the vicinity of vacancies, yellow spheres 
    depict twin/screw dislocations, and black spheres highlight 
    unidentified defect atoms.
    The nucleation and propagation of edge dislocations on the 
    \{111\} slip 
    family are observed, which then evolve into prismatic loops.
    In addition, identified slip traces and pile-ups are well 
    modeled by NNIP 
    simulations showing the well--known three-fold symmetric 
    rosette depths below 1.45 nm that are 
    formed by [11$\Bar{2}$], [$\Bar{1}$01] and [0$\Bar{1}$1] 
    planes. }
    \label{fig:bda_method}
\end{figure}


==> sections/discussions.tex <==
\section{\label{sec:discussion} Discussion 
and conclusions
} 
Interatomic potentials developed before the present work, 
although adequate for many applications, need to be improved for nanoindentation simulations. For example, J. Byggmästar {\em et. al.}~\cite{dataset} developed a GAP potential for Mo, demonstrating accuracy and transferability for elastic, thermal, liquid, defect, and surface properties. However, this potential failed to produce reliable data for the shear stress in the elastic region in the early stages of the nanoindentation simulation. Furthermore, in contrast to the NNIP developed here, 
many prismatic loops were nucleated during the nanoindentation (see Fig. \ref{fig:bda_method}), potentially due to insufficient information in the energy landscape regarding the dislocation cores, a fact that was illustrated based on the similarity of the GSF configurations with the dislocation cores as depicted in Fig. \ref{fig:GSFE}. 

The tabGAP potentials are designed for complex multi-element materials \cite{PhysRevMaterials.6.083801}, employing simple low-dimensional descriptors. Although tabGAP potentials have notable accuracy for entropy alloys \cite{PhysRevB.104.104101}, the same issues as the GAP potential arise when it comes to single element BCC Mo. As mentioned earlier, the tabGAP potential leads to nucleation of too 
many prismatic dislocation loops in the nanoindentation simulations (see Fig. \ref{fig:bda_method})
Moreover, accurate predictions of shear stress in the initial phases of the nanoindentation simulations were not achieved. 

The EAM/FS potential utlized in this study~\cite{ESalonen_2003}, originally designed for radiation damage simulations, failed to accurately produce GSFE curve for Mo in both pristine crystalline and GSF configurations representing dislocation cores. Consequently, it is 
unclear whether or not 
this potential can reliably predict dislocation nucleation during indentation. In addition, similar to the other potentials, it does not correctly predict the shear stress.

Considering the challenges faced in nanoindentation simulations, the presence of a well-developed methodology to tackle these issues would be highly beneficial. 
In this work, we met this goal by introducing to the training dataset
new configurations which  resemble the local atomic environments of an indented sample. 
The similarity measurements presented here ensure the relevance of the newly introduced structures to a nanoindentation simulation. 
To the best of our knowledge, this study represents the first attempt to develop a machine-learnt interatomic potential specifically 
designed for nanoindentation simulations.  
The novel configurations 
introduced here
could aid the development of
ML potentials for other materials. 
